Differentially Private Federated Knowledge Graphs Embedding

Knowledge graph embedding plays an important role in knowledge representation, reasoning, and data mining applications. However, for multiple cross-domain knowledge graphs, state-of-the-art embedding models cannot make full use of the data from different knowledge domains while preserving the privacy of exchanged data. In addition, the centralized embedding model may not scale to the extensive real-world knowledge graphs. Therefore, we propose a novel decentralized scalable learning framework, \emph{Federated Knowledge Graphs Embedding} (FKGE), where embeddings from different knowledge graphs can be learnt in an asynchronous and peer-to-peer manner while being privacy-preserving. FKGE exploits adversarial generation between pairs of knowledge graphs to translate identical entities and relations of different domains into near embedding spaces. In order to protect the privacy of the training data, FKGE further implements a privacy-preserving neural network structure to guarantee no raw data leakage. We conduct extensive experiments to evaluate FKGE on 11 knowledge graphs, demonstrating a significant and consistent improvement in model quality with at most 17.85\% and 7.90\% increases in performance on triple classification and link prediction tasks.

==> Model.tex <==
\section{Federated Knowledge Graphs Representation Learning}\label{sec:model}
In this section, we present detailed descriptions of FKGE.
We define the set of knowledge graphs from separate owners as $\mathcal{KG} = \{g_1, g_2, g_3, ..., g_D\}$, where $D$ is the total number of knowledge graphs and $g_k = \{\mathcal{E}_k, \mathcal{R}_k, \mathcal{T}_k\} (1 \leq k \leq D)$ indicates the $k$-th knowledge graph. Each triple $(h,r,t) \in \mathcal{T}_k$ (the set of triples of $g_k$) is composed of a head entity $h \in \mathcal{E}_k$ (the set of entities of $g_k$), a tail entity $t \in \mathcal{E}_k$ and a relation $r \in \mathcal{R}_k$ (the set of relations of $g_k$).
Following the OpenKE \cite{openke}, our FKGE is compatible with various KGE models as base embedding models.
Based on the embeddings trained by base models, FKGE aggregates the embeddings of both aligned and added entities and relations from paired knowledge graphs and retrain embeddings in the federal units.
For aligned entities and relations from a pair of knowledge graphs, e.g., $(g_i, g_j)$, our goal is to construct a secure pipeline that can refine the embeddings of $\mathcal{E}_i \cap \mathcal{E}_j$ and $\mathcal{R}_i \cap \mathcal{R}_j$.


\subsection{Privacy-Preserving Adversarial Model}
To refine embeddings of aligned entities and relations from paired knowledge graphs in different domains, we implement a privacy-preserving pairwise GAN (AIR-GAN) inspired by MUSE~\cite{gan_translation}, which is used for multilingual word embedding translation.
For any pair of $(g_i, g_j)$, the architecture of our pairwise GAN is illustrated in Figure~\ref{GAN}.
The generator $G$ with parameters $\theta_G$ locates in $g_i$'s database while discriminator $D$ with parameters $\theta_D$ lies in $g_j$'s database. 
We define $g_j$ as host and $g_i$ as client, since the host is responsible for both generator and discriminator loss backpropagation calculations and client only transmits its generator output and receives gradients to update its own parameters. 
We use $X=\{x_1,x_2,...,x_n\}$ to denote embeddings for $\mathcal{E}_i \cap \mathcal{E}_j$ and $\mathcal{R}_i \cap \mathcal{R}_j$ in $g_i$, and $Y=\{y_1,y_2,...,y_n\}$ to denote embeddings for $\mathcal{E}_i \cap \mathcal{E}_j$ and $\mathcal{R}_i \cap \mathcal{R}_j$ in $g_j$.
The objective of generator $G$ is to generate adversarial samples by making $G(x_i)$ and $y_i$ similar under the CSLS metric used by MUSE \cite{gan_translation}, while discriminator $D$ focuses on classifications between fake samples $G(X)$ and real samples $Y$.
%We add adjacent entities of $X$ and joined relations as anonymous virtual entities and relations into the vector space of $g_j$ to improve training performance.
%The virtual entities and relations receive embeddings from the generator and are only used for knowledge graph embedding training as fake data that will be dumped after retraining.
The loss function is formulated as:


\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{SGAN}
\caption{The architecture of privacy-preserving adversarial model. The host and client are separated: only adversarial examples and gradients from the discriminator are exchanged, maintaining all raw data and embedding in private.}\label{GAN}
\end{figure}


\begin{algorithm}[t]
{\footnotesize
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\SetAlgoLined
\KwInput{$g_j$. the Host KG}
\KwOutput{Best embedding}
$best\ embedding \leftarrow train(g_j)$\;
$best\ score \leftarrow test(best\ embedding)$\;
$g_j.state \leftarrow Ready$\;
\tcc{Q is handshake signal Queue of $g_j$}
$Q.receive\_signal()$ \tcc*[r]{receiving signal as Host}
\While{$g_j.state = Ready$}     
{
    $improved \leftarrow False$\;
    \While{$Q\ is\ not\ empty$}
    {
        $g_j.state = Busy$\;
        $translated\ embedding \leftarrow Active\_handshake(g_j,\ Q.poll())$\;
        $aggregation(g_j, translated\ embedding)$\;
        $embedding \leftarrow retrain(g_j)$\;
        $score \leftarrow test(embedding)$\;
        \tcc{backtrack function is the embodiment of our backtrack mechanism} 
        $improved,\ best\ score,\ best\ embedding \leftarrow backtrack(score,\ best\ score,\ embedding,\ best\ embedding)$;\\
        $g_j.state = Ready$\;
    }
    \If{$improved\ =\ False\ \textbf{and}\ Q\ is\ empty$}{
        \tcc{both following states is configured by KG owner or activated by handshake signal}
        \If{$g_j.state = Sleep$}{
                $g_j.sleep()$\;
        }
        \If{$g_j.state = Ready$}{
            \tcc{$g_j$ begins self iterative training}
           $embedding \leftarrow train(g_j)$\;
            $score \leftarrow test(embedding)$\;
            $improved,\ best\ score,\ best\ embedding \leftarrow backtrack(score,\ best\ score,\ embedding,\ best\ embedding)$;\\
        }
    }
    \If{$improved\ = True\ \textbf{and}\ Q\ is\ empty$}{
    \tcc{broadcast handshake signal to KGs having aligned entities and relations}
          $g_j.send\_handshake\_signal(\mathcal{KG})$\;
    }
}
\Return $best\ embedding$\;
}
 \caption{KG processor} \label{processor}
\end{algorithm}



\textbf{Generator Loss:}
\begin{equation}
L_G(\theta_G | D) = -\frac{1}{n} \sum_{i=1}^{n} [log P_{\theta_D}(D(G(x_i)) = 1)
+log P_{\theta_D}(D(y_i) = 0)].
\end{equation}
 
\textbf{Discriminator Loss:}
%\begin{equation}
%L_D(\theta_D | G) = -\frac{1}{n} \sum_{i=1}^{n} log P_{\theta_D}(D(G(x_i)) = 0)
%-\frac{1}{n} \sum_{i=1}^{n} log P_{\theta_D}(D(y_i) = 1)
%\end{equation}
\begin{equation}
L_D(\theta_D | G) = -\frac{1}{n} \sum_{i=1}^{n} [log P_{\theta_D}(D(G(x_i)) = 0)
+log P_{\theta_D}(D(y_i) = 1)].
\end{equation}
%privacy concerns

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{Framework}
\caption{An example of whole training procedure.
The order of training is not fixed and depends on individual knowledge graph owner's computation power and willingness to cooperate.
``Train'' indicates training Knowledge Graph Embedding Model locally. 
``Trans i-j'' denotes the pairwise GAN model translating embeddings between $g_i$ and $g_j$ where generator locates in client $g_i$ and discriminator lies in host $g_j$. 
``Agg'' exploits replacement and addition to refine embeddings of $g_j$.
If result of host $g_j$ has more accurate representation than previous embedding, the result is stored and then the $g_j$ broadcasts signal to other knowledge graphs for further aggregations.
Otherwise the result is backtracked.
State switch line indicates the state switch to ready or sleep state.
}\label{frame}
\end{figure*}


To guarantee data security during interactions between knowledge graphs from isolated databases, our model ensures no raw data leakage. 
The raw embeddings of aligned entities and relations in $X$ are fed to generator to generate adversarial samples $G(X)$ which are later on transmitted to discriminator $D$.
The raw embeddings of aligned entities and relations in $Y$ and $G(X)$ are fed to discriminator which aims to distinguish $Y$ as real data and $G(X)$ as fake data.
During the training process, the discriminator calculates both generator and discriminator loss functions locally: gradients from discriminator loss are used to update discriminator parameters locally while gradients from generator loss calculated in discriminator are sent back to generator to update its parameters.
Therefore, neither of $g_i$ and $g_j$ is able to access the embeddings or raw data of the other's. The sensitive data security and privacy are protected for any participant of knowledge graph owners. 


In addition to the generated embedding $G(X)$, after the pairwise GAN is stable, the client generates embeddings for the adjacent entities of the aligned entities in $g_i$ and the joining relations as types of virtual entities and relations that are added into the host.
We use $N(X)$ to denote the raw embeddings of adjacent entities and joining relations in $g_i$, and the generated embeddings of virtual entities and relations can be denoted as $G(N(X))$.
These virtual entities and relations are only used for KGE, and will be removed before responding to other hosts.

%For adjacent entities of $X$ and relations joining $X$, we add their generated embeddings into embedding space of $g_j$ as virtual entities and relations.
%These virtual entities and relations are only used for knowledge graph training, and will be dumped after retraining.



\subsection{Federated Training}
For multiple knowledge graphs, we construct pairwise GANs between any pair of $(g_i, g_j) \in \mathcal{KG}$ where $\mathcal{E}_j \cap  \mathcal{E}_i \neq \emptyset$ or $\mathcal{R}_j \cap  \mathcal{R}_i \neq \emptyset$, and produce $2\times\binom{D}{2}$ pairwise GANs at most in the same time. 
For any pair of $(g_i,g_j)$, at least one generator and one discriminator are required separately. 
Our asynchronous and decentralized setting allows individual knowledge graph owner to decide whether it should collaborate with other knowledge graphs.
More specifically, the collaboration process could be described as a handshake protocol. 
Any $g_i$ has three states: ready, busy and sleep.
Ready state indicates $g_i$ having available computational resources and being active to pair up with other knowledge graphs. 
Busy state indicates that $g_i$ does not have enough resources and will not respond to any collaboration request at the moment. Instead, collaborators will be put in a queue till $g_i$ finishes its work and is ready for collaborations.
Sleep state indicates that though $g_i$ has the computational resources, it has not received any collaboration request yet. That is, If ready state could not find a partner, it will switch to sleep state and wake up to ready state after a certain time period or being notified by a collaboration request.
Algorithm \ref{processor} describes how a knowledge graph refines its embeddings.
A successful handshake process between $g_i$ and $g_j$ implies $state(g_i) \neq busy, state(g_j) \neq busy $, and at least one of them has ready state.



Figure~\ref{frame} illustrates an example of federated training process. 
Every knowledge graph needs to train its embedding model locally, the objective is to generate more accurate representation than previous input. 
The red lines denote successful handshake processes.
For one round of federated training, two knowledge graphs begin with a handshake signal.
After establishing a stable connection between collaborators in a pair, the pairwise GAN is trained immediately with one host $g_j$ and one client $g_i$. 

\begin{algorithm}[t]
{\footnotesize
%\SetAlgoNoLine
\SetKwInOut{KIN}{Input}
\SetKwInOut{KOUT}{Output}
%\BlankLine
    \caption{Active\_handshake}
    \label{DE_algo} %
    \KIN{$g_j$, Host KG, $g_i$, Client KG}
    \KOUT{Translated embedding}   
    \tcc{the caller is the $g_j$, Host KG.}
    $construct\ pairwise\ GAN\ between\ g_i\ and\ g_j$\;
    \Repeat{$GAN\ processing\ finished$}{
        $adversarial\ samples \leftarrow g_i.generate(X)$\;
        $g_j.receive(g_i.send(adversarial\  samples))$\tcc*[r]{communication between processes}
        $probability\leftarrow g_j.discriminator(Y,\ adversarial\ samples)$\;
        $loss\_gen,\ loss\_dis \leftarrow g_j.loss\_function(probability)$\;
        $gradient\_generator,\ gradient\_discriminator \leftarrow backpropagation(loss\_gen,\ loss\_dis)$\;
        $g_i.receive(g_j.send(\ gradient\_generator))$ \tcc*[r]{communication between processes}
        $g_j.update\_parameters(\ \Theta_D, gradient\_discriminator)$\;
        $g_i.update\_parameters(\ \Theta_G, gradient\_generator)$\;
    }
    $translated\ embedding \leftarrow g_j.receive(g_i.send(adversarial\ samples, g_i.generate(N(X))))$\tcc*[r]{communication between processes}
    \Return $translated\ embedding$\;
}
\end{algorithm}


As described in last subsection, after the training process, the client will send its $G(X)$ and $G(N(X))$ to the host, and the host will run aggregation algorithms including replacement (replace embeddings of aligned entities and relations in $Y$ with $G(X)$) and addition (add $G(N(X))$ into $Y$).
Then both overlapped and added embeddings of host are refined, overall embeddings of the host are fed to train locally. 
If output embeddings are more accurate than previous embeddings, the knowledge graph embedding is then replaced by the better embeddings and since embeddings of the host are improved, the host will switch to ready state and actively seek other KGs with overlapped entities and relations for next round of federated training.
On the contrary, if the output embeddings give poorer results compared with previous knowledge graph embedding, we abandon the poor embeddings and backtrack to previous embeddings.
If host has already finished training with all KGs with overlapped entities and relations and failed to achieve better performance, it will then turn to sleep or ready state by individual setting, and wait for overlapped knowledge graphs with refined embeddings to start new rounds of federated training.
In addition, if the host still has collaborators in its queue, the host will switch to ready state and actively start new federated training with these queued collaborators.


Every time embeddings of $g_j$ are improved, we broadcast them to collaborators to start federated training since each refined embedding may further improve other collaborators' embeddings.
When a knowledge graph acts as a host, it will not accept any host role even computational resources are available.
The host puts such requests in a queue and will handshake with them in a first come first serve basis later.
The whole handshake mechanism is explained in Algorithm~\ref{DE_algo}.
